Social Conjuring: Multi-User Runtime Collaboration with AI in Building Virtual 3D Worlds

Generative artificial intelligence has shown promise in prompting virtual worlds into existence, yet little attention has been given to understanding how this process unfolds as social interaction. We present Social Conjurer, a framework for AI-augmented dynamic 3D scene co-creation, where multiple users collaboratively build and modify virtual worlds in real-time. Through an expanded set of interactions, including social and tool-based engagements as well as spatial reasoning, our framework facilitates the creation of rich, diverse virtual environments. Findings from a preliminary user study (N=12) provide insight into the user experience of this approach, how social contexts shape the prompting of spatial environments, and perspective on social applications of prompt-based 3D co-creation. In addition to highlighting the potential of AI-supported multi-user world creation and offering new pathways for AI-augmented creative processes in VR, this article presents a set of implications for designing human-centered interfaces that incorporate AI models into 3D content generation.

==> images/scene_examples/scene-examples.tex <==
% \begin{figure}[ht]
%   \centering
%   \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/scene examples/zoo-cropped.png}
%     \caption{Scene generated by the prompt \textit{"create a zoo"}}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/scene examples/amusement-park-cropped.png}
%     \caption{Scene generated by the prompt \textit{"create an amusement park at night"}}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/scene examples/fantasy-forest-cropped.png}
%     \caption{Scene generated by the prompt "create a fantasy forest" and "add a unicorn and gnome", and modifed with tools.}
%   \end{subfigure}
  
%   \caption{Sample tools and tool output generated by our system.}
%   \label{fig:scene-examples}
%   \vspace{-6mm}
% \end{figure}

\begin{figure}[ht]
  \centering
  \begin{subfigure}[t]{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/scene_examples/zoo-cropped.png}
    \caption{Scene generated by the prompt \textit{"create a zoo"}.}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/scene_examples/amusement-park-cropped.png}
    \caption{Scene generated by the prompt \textit{"create an amusement park at night"}.}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/scene_examples/fantasy-forest-cropped.png}
    \caption{Scene generated by the prompts \textit{"create a fantasy forest"} and \textit{"add a unicorn and gnome,"} and modified with tools.}
  \end{subfigure}
  
  \caption{Examples of scenes generated by Conjurer.}
  \label{fig:scene-examples}
  \vspace{-6mm}
\end{figure}



==> tables/dataset-distribution-table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Spatial Relationship} & \textbf{Count} \\ \hline
Above  & 164  \\ \hline
Behind & 111  \\ \hline
Below  & 161  \\ \hline
Front  & 111  \\ \hline
Left   & 146  \\ \hline
Right  & 147  \\ \hline
\end{tabular}
\caption{Distribution of Spatial Relationships}
\label{tab:spatial-relationships}
\end{table}

